Improved Fermion Hamiltonians for Quantum Simulation

We developed a Hamiltonian inspired by ASQTAD and highly improved staggered quark (HISQ) actions and show how these Hamiltonians can be used for quantum simulations. Gate costs for the time evolution of these improved Hamiltonians are provided as well as a demonstration of the reduction of lattice spacing errors using the 1+1d lattice Schwinger model.

==> hisq.tex <==
\section{HISQ}
\begin{enumerate}
    \item Issues with ASQTAD action / Hamiltonian
    \begin{enumerate}
        \item While the ASQTAD Hamiltonian addresses the issue of Tree level $\mathcal{O}(a^2)$ effects. There are still errors of $\mathcal{O}(\alpha_s a^2)$ which are crucially important.
        \item In the action formalism this was addressed by implementing a second level of ASQTAD smearing after reunitarizing the gauge links.
        \item This resulted in the highly improved staggered quark (HISQ) action. CITE SOME STUFF HERE
    \end{enumerate}
    \item The HISQ Hamiltonian
    \begin{enumerate}
        \item The HISQ Hamiltonian Kinetic term will be
        \begin{equation}
            \label{eq:hamhisq}
            \begin{split}
            H^{HISQ}_{kinetic} = &\frac{1}{2a} \sum_{\vec{r}}\sum_{m} \bigg\lbrace \xi_{m}(\vec{r}) \phi^{\dagger}(\vec{r}) \Big( \hat{W}_m(\vec{r}) \phi(\vec{r} + \hat{m}) \\ & -\frac{1}{24} \hat{X}_m(\vec{r})\hat{X}_m(\vec{r}+\hat{m})\hat{X}_m(\vec{r}+2\hat{m})\phi(\vec{r}+3\hat{m})\Big) + h.c.\bigg\rbrace
            \end{split}
        \end{equation}
        \item where
        \begin{equation}
            \label{eq:HISQW}
            \hat{W}_m(\vec{r}) = \mathcal{R}[\mathcal{F}^{HISQ}[\hat{U}_m(\vec{r})]],
        \end{equation}
        \begin{equation}
            \hat{X}_m(\vec{r}) = \mathcal{R}[\mathcal{F}^{(1)}[\hat{U}_m(\vec{r})]]
        \end{equation}
        and
        \begin{equation}
            \mathcal{F}^{HISQ}[\hat{U}_m(\vec{r})] = \Big(\mathcal{F}^{(1)}[\mathcal{R}[\mathcal{F}^{(1)}[\hat{U}_m(\vec{r})]]] - 2 \mathcal{F}^{(2)}[\mathcal{R}[\mathcal{F}^{(1)}[\hat{U}_m(\vec{r})]]]\Big)
        \end{equation}
    \end{enumerate}
\end{enumerate}

